DeepDPM: Deep Clustering With an Unknown Number of Clusters

Deep Learning (DL) has shown great promise in the unsupervised task of clustering. That said, while in classical (i.e., non-deep) clustering the benefits of the nonparametric approach are well known, most deep-clustering methods are parametric: namely, they require a predefined and fixed number of clusters, denoted by K. When K is unknown, however, using model-selection criteria to choose its optimal value might become computationally expensive, especially in DL as the training process would have to be repeated numerous times. In this work, we bridge this gap by introducing an effective deep-clustering method that does not require knowing the value of K as it infers it during the learning. Using a split/merge framework, a dynamic architecture that adapts to the changing K, and a novel loss, our proposed method outperforms existing nonparametric methods (both classical and deep ones). While the very few existing deep nonparametric methods lack scalability, we demonstrate ours by being the first to report the performance of such a method on ImageNet. We also demonstrate the importance of inferring K by showing how methods that fix it deteriorate in performance when their assumed K value gets further from the ground-truth one, especially on imbalanced datasets. Our code is available at https://github.com/BGU-CS-VIL/DeepDPM.

==> macros.tex <==
 %--------------------------------------------
% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
% \def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
% \def\wrt{with respect to }  % The extra space at the end means \wrt blah would 
% not end up as ``with respect toblah''. 
 
\def\dof{d.o.f\onedot}
% \def\etal{\emph{et al}\onedot}
\def\etal{\emph{et al}\onedot}
% \def\etal{\emph{et al}\onedot}
%
\def\iid{\emph{i.i.d}\onedot}
% \def\pdf{\emph{p.d.f}\onedot}



\makeatother
%--------------------------------------------------

\newcommand{\FIG}{Fig.~}
\newcommand{\FIGS}{Figs.~}
\newcommand{\EQN}{Eq.~}
% \newcommand{\EQN}{Equation }
\newcommand{\EQNS}{Eqs.~}
% \newcommand{\EQNS}{Equations }

%\newcommand{\SEC}{Sec.~}.  Use \autoref or ~\autoref instead.



% integers
\newcommand{\ZZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\RR}{\ensuremath{\mathbb{R}}}
\newcommand{\Rtwo}{\ensuremath{\RR^2}}
\newcommand{\Rthree}{\ensuremath{\RR^3}}
\newcommand{\Rfive}{\ensuremath{\RR^5}}

\newcommand{\Rsix}{\ensuremath{\RR^6}}

\newcommand{\Rn}{\ensuremath{\RR^n}}
\newcommand{\Rd}{\ensuremath{\RR^d}}
\newcommand{\RD}{\ensuremath{\RR^D}}
\newcommand{\Rk}{\ensuremath{\RR^k}}

% 
%positive integers
\newcommand{\Zplus}{\ensuremath{\ZZ^+}}
%positive reals
\newcommand{\Rplus}{\ensuremath{\RR^+}}


% set notation
% \newcommand{\set}[1]{\ensuremath{{\left\{#1\right\}}}}
\newcommand{\set}[1]{\ensuremath{{\{#1\}}}}
\newcommand{\tuple}[1]{\ensuremath{{(#1)}}}
\newcommand{\tupleLarge}[1]{\ensuremath{{\left(#1\right)}}}
\newcommand{\argmin}[1]{\ensuremath{\operatorname*{arg\,min}_{#1}}}
\newcommand{\argmax}[1]{\ensuremath{\operatorname*{arg\,max}_{#1}}}



\newcommand{\InnerProduct}[2]{\left\langle #1,#2 \right\rangle}

\newcommand{\norm}[1]{{{\left\|#1\right\|}}}
\newcommand{\sign}[1]{{\mathrm{sign}\left(#1\right)}}

\newcommand{\ellTwo}{\ell_2}
\newcommand{\ellTwoNorm}[1]{\norm{#1}_{\ellTwo}}
\newcommand{\ellOne}{\ell_1}




\newcommand{\MATRIX}[2][cccccccccccccccccccc]{\left[
 \begin{array}{#1}
 #2
 \end{array}
\right]}

\newcommand{\Mod}[1]{\ (\mathrm{mod}\ #1)}



% homogeneous coordinates
\newcommand{\bxh}{\widetilde{\bx}}
\newcommand{\WHITE}[1]{{{\color{white}{#1}}}}  

\newcommand{\RED}[1]{{{\color{red}{#1}}}}  
\newcommand{\BLUE}[1]{{{\color{blue}{#1}}}}
\newcommand{\GREEN}[1]{{{\color{green}{#1}}}}
\newcommand{\MAGENTA}[1]{{{\color{magenta}{#1}}}}  

\definecolor{brown}{RGB}{165,42,42}
\newcommand{\BROWN}[1]{{{\color{brown}{#1}}}}



\newcommand{\FREIFELD}[1]{\textbf{\MAGENTA{[FREIFELD says: #1]}}}
\newcommand{\MEITAR}[1]{\textbf{\BLUE{[MEITAR says: #1]}}}
\newcommand{\SHAHF}[1]{\textbf{\GREEN{[SHAHAF says: #1]}}}
% Make your own

\newcommand{\TBD}{\RED{[TBD]}}
\newcommand{\TODO}[1]{\RED{[TODO: #1]}}
\newcommand{\REPLACE}[2]{\RED{REPLACE:} \BLUE{#1} \RED{WITH:} \BLUE{#2}}



% In python: print_iterable(['\\bmdefine\\b{0}'.format(x)+'{'+x+'}' for x in 
% string.ascii_letters])

\bmdefine\ba{a}
\bmdefine\bb{b}
\bmdefine\bc{c}
\bmdefine\bd{d}
\bmdefine\be{e}
% \bmdefine\bf{f}  # Clashes with a standard command
\bmdefine\boldf{f}
\bmdefine\bg{g}
\bmdefine\bh{h}
\bmdefine\bi{i}
\bmdefine\bj{j}
\bmdefine\bk{k}
\bmdefine\bl{l}
\bmdefine\bm{m}
\bmdefine\bn{n}
\bmdefine\bo{o}
\bmdefine\bp{p}
\bmdefine\bq{q}
\bmdefine\br{r}
\bmdefine\bs{s}
\bmdefine\bt{t}
\bmdefine\bu{u}
\bmdefine\bv{v}
\bmdefine\bw{w}
\bmdefine\bx{x}
\bmdefine\by{y}
\bmdefine\bz{z}
\bmdefine\bA{A}
\bmdefine\bB{B}
\bmdefine\bC{C}
\bmdefine\bD{D}
\bmdefine\bE{E}
\bmdefine\bF{F}
\bmdefine\bG{G}
\bmdefine\bH{H}
\bmdefine\bI{I}
\bmdefine\bJ{J}
\bmdefine\bK{K}
\bmdefine\bL{L}
\bmdefine\bM{M}
\bmdefine\bN{N}
\bmdefine\bO{O}
\bmdefine\bP{P}
\bmdefine\bQ{Q}
\bmdefine\bR{R}
\bmdefine\bS{S}
\bmdefine\bT{T}
\bmdefine\bU{U}
\bmdefine\bV{V}
\bmdefine\bW{W}
\bmdefine\bX{X}
\bmdefine\bY{Y}
\bmdefine\bZ{Z}


\bmdefine\balpha{\alpha}
\bmdefine\bbeta{\beta}
\bmdefine\bgamma{\gamma}

\bmdefine\bdelta{\delta}
\bmdefine\btheta{\theta}
\bmdefine\blambda{\lambda}
\bmdefine\bphi{\phi}
\bmdefine\bxi{\xi}
\bmdefine\bzeta{\zeta}
\bmdefine\boldeta{\eta}
\bmdefine\bpi{\pi}

\bmdefine\bmu{\mu}
\bmdefine\brho{\rho}
\bmdefine\bomega{\omega}
\bmdefine\bOmega{\Omega}
\bmdefine\bPi{\Pi}

\bmdefine\bvarepsilon{\varepsilon}
\bmdefine\bepsilon{\epsilon}


\bmdefine\bDelta{\Delta}

\bmdefine\bTheta{\Theta}

\bmdefine\bsigma{\sigma}
\bmdefine\bSigma{\Sigma}
\bmdefine\bPsi{\Psi}
\bmdefine\bLambda{\Lambda}



\bmdefine\bzero{0}
\bmdefine\bone{1}
\bmdefine\binfty{\infty}

 \newcommand{\indicator}{\mathbbm{1}}


% In python 
% print_iterable(['\\newcommand{\\'+'{0}cal'.format(x)+'}{\\mathcal{'+x+'}}' 
% for x in string.ascii_uppercase])
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}


 \newcommand{\DP}{\mathrm{DP}}
 \newcommand{\DIR}{\mathrm{Dir}}
 \newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%


==> supmat/not_used/my_ablations_test.tex <==
\begin{table}[h]
\centering
%\resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}m{3.755cm} m{1.15cm}m{1.29cm}m{1.29cm}@{}}
    \toprule
 & \multicolumn{3}{c}{ACC}\\
    \midrule
    & $K_\mathrm{init}$=3 & $K_\mathrm{init}$=10 &$K_\mathrm{init}$=30\\
    \midrule
    \hline
    No splits/merges & .29$\pm$.01 & .59$\pm$.03 & .46$\pm$.01\\
    No splits & .29$\pm$.01 & .59$\pm$.02 & .45$\pm$.03\\
    No merges & .46$\pm$.00 & .58$\pm$.01 & .47$\pm$.01 \\
    2-means instead of $f_{\mathrm{sub}}$
    %subclusters nets
    & .61$\pm$.00 & .59$\pm$.02 & .56$\pm$.02 \\
%     No priors 
    No priors in the $M$ step
    & .58$\pm$.01 & .57$\pm$.02 & .58$\pm$.01 \\
    Isotropic loss instead of $\Lcal_{\mathrm{cl}}$ & .58$\pm$.01 & .58$\pm$.02 & .57$\pm$\TBD \\
	%subcluster loss KL & .59$\pm$.03 & .59$\pm$.01 & .58$\pm$.03 \\
	%$\alpha$ = 0.1 & .59$\pm$.01 & \TBD & \TBD\\
	%$\alpha$ = 1 & .59$\pm$.06 & \TBD & \TBD\\
	%$\alpha$ = 100 & \TBD & \TBD & \TBD\\
	DeepDPM (full method) & \textbf{.62$\pm$.03} & \textbf{.61$\pm$.00} & \textbf{.62$\pm$.01}\\  
    \bottomrule
    \end{tabular}%
    %}
\caption[Ablations]{DeepDPM's performance under different ablations.}
\label{results:DPM_ablations}
\end{table}


==> supmat/not_used/results_files/comp_classical/final_K_imbalanced.tex <==
\begin{figure}
\centerline{\includegraphics[scale=.4]{./Imbalanced_K.pdf}}
\caption[Comparing final K]{Comparing the inferred value of $K$ for methods which find it in imbalanced datasets. For all datasets, ground truth $K$ is 10. The dots are the mean result of 10 independent runs and the bars are the standard deviation.}
\label{results_figs:final_K_imbalanced}
\end{figure}

==> supmat/not_used/results_files/datasets.tex <==
\section{Datasets}
\input{./results_files/Datasets/datasets_summary}

We evaluate and compare our approach on the following datasets, also summarized in Table~\ref{results:datasets}.
\begin{itemize}
	\item \textbf{MNIST}~\cite{Datasets:Deng:2012:MNIST}. An image dataset that has 70,000 data samples. Each sample is a 28 $\times$ 28 gray-scale image containing a handwritten digit, i.e., one of {0, 1, \dots , 9}. A number of samples from this dataset can be seen in~\autoref{datasets:mnist}.
	\input{./results_files/Datasets/MNIST_fig}
	\item \textbf{USPS~\cite{Datasets:USPS}}. An image dataset that has 9298 samples. Each sample is a 16 $\times$ 16 gray-scale image containing a handwritten digit. A few examples of this dataset can be seen in~\autoref{datasets:usps}.
	\input{./results_files/Datasets/USPS_fig}
	\item \textbf{Fashion-MNIST~\cite{Datasets:Xiao:2017:FashionMNIST}}. An MNIST-like dataset of 70,000, 28 $\times$ 28 gray-scale image labelled fashion images.
	 Some random images from this dataset can be seen in~\autoref{datasets:fashionMNIST}.
	\input{./results_files/Datasets/FashionMNIST_fig}
	\item \textbf{STL-10~\cite{Datasets:Coates:2010:STL10}}. An image dataset of 96-by-96 color images. There
are 10 classes with 1300 examples each. While it also contains 100000 unlabeled images of the same resolution, we used only the labelled samples for training for a fair comparison with the algorithms that cannot scale to the full dataset. See~\autoref{datasets:stl10} for examples.
\input{./results_files/Datasets/STL10_fig}
	\item \textbf{Reuters10k} Reuters dataset~\cite{Datasets:Lewis:2004:reuters} contains about 810000 English news stories labelled with a category tree. We followed the framework suggested by~\cite{DC:Xie:2016:DEC} and used the four root categories: corporate/industrial, government/social, markets, and economics as labels and further pruned all documents that are labelled by multiple root categories to get 685071 articles. We then computed tf-idf features on the 2000 most frequently occurring word stems. Since, unlike our method, some of the competing algorithms do not scale to the full Reuters dataset, we 
%also
sampled a random subset of 10000 examples, which we call REUTERS-10k, for comparison purposes.
\end{itemize}


==> theorems.tex <==
\theoremstyle{definition}  
% \theoremsymbol{\scalebox{1}[1.4]{\large$ \diamond $}}
\newtheorem{Definition}{Definition}
\newtheorem{Example}{Example}
\newtheorem{Theorem}{Theorem}
\newtheorem*{Proof}{Proof}
\newtheorem{Remark}{Remark}

